Do Compressed LLMs Forget Knowledge? An Experimental Study with Practical Implications

Compressing Large Language Models (LLMs) often leads to reduced performance, especially for knowledge-intensive tasks. In this work, we dive into how compression damages LLMs' inherent knowledge and the possible remedies. We start by proposing two conjectures on the nature of the damage: one is certain knowledge being forgotten (or erased) after LLM compression, hence necessitating the compressed model to (re)learn from data with additional parameters; the other presumes that knowledge is internally displaced and hence one requires merely "inference re-direction" with input-side augmentation such as prompting, to recover the knowledge-related performance. Extensive experiments are then designed to (in)validate the two conjectures. We observe the promise of prompting in comparison to model tuning; we further unlock prompting's potential by introducing a variant called Inference-time Dynamic Prompting (IDP), that can effectively increase prompt diversity without incurring any inference overhead. Our experiments consistently suggest that compared to the classical re-training alternatives such as LoRA, prompting with IDP leads to better or comparable post-compression performance recovery, while saving the extra parameter size by 21x and reducing inference latency by 60%. Our experiments hence strongly endorse the conjecture of "knowledge displaced" over "knowledge forgotten", and shed light on a new efficient mechanism to restore compressed LLM performance. We additionally visualize and analyze the different attention and activation patterns between prompted and re-trained models, demonstrating they achieve performance recovery in two different regimes.

==> figures/cosim_opt.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=0.8\linewidth]{images/Cossim_opt.pdf} % replace with your actual image filename
\caption{Quantized OPT-7b layer-wise's attention and activation similarity to baseline using various PEFT methods. }
\label{fig:cos_opt}
\end{figure}

==> figures/peft_sparsegpt_perf.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=0.8\linewidth]{images/PEFT_performance_sparseGPT_V2.pdf} % replace with your actual image filename
\caption{GPTQ LLama-7b/OPT-6.7b average accuracy across nine tasks vs. number of trainable parameters of various PEFT methods on C4/Wikitext finetune dataset. Prompts exhibits far higher performance consistency and task performance with lower overall cost.  }
\label{fig:sparse}
\end{figure}

==> figures/sneakpeak.tex <==
\begin{figure}[hbpt]
 % \vspace{-10pt}
\centering
\includegraphics[width=0.9\linewidth]{images/performance_overview.pdf} 
\vspace{-8pt}
\caption{Performance comparison of various tuning techniques on a compressed 3-bit Llama-7b. dash-line indicates baseline performance. Our technique has the highest average accuracy for nine different tasks. }
% \vspace{-7pt}
\label{fig:sneakpeak}
\end{figure}

==> tables/gptq_c4.tex <==


\begin{table}
\caption{Average accuracy for nine seperate tasks across three separate runs for various adaptation method of 3 bit GPTQ quantized models.}
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{lllll|rrrrrrrrr|r}
\toprule
model & type & task & tokens & r & arcC & arcE & hellaswag & lambada & piqa & sciq & triviaqa & webqs & winogrande & avg\_acc \\
\midrule
opt-6.7b & --- & --- & --- & --- & 29.01 & \textbf{64.77}& 48.57 & 65.34 & 75.24 & 89.40 & 17.90 & 9.50 & \textbf{63.54} & 51.47 \\
opt-6.7b & ptune & c4 & 12 & --- & 29.01 & 62.70 & 48.26 & 64.52 & 75.51 & 88.33 & 18.22 & 10.50 & 61.17 & 50.91 \\
opt-6.7b & ptune & c4 & 25 & --- & 28.92 & 62.75 & 48.43 & 64.81 & 75.43 & 88.80 & 18.09 & 10.15 & 61.33 & 50.97 \\
opt-6.7b & ptune & c4 & 50 & --- & 28.98 & 62.81 & 48.43 & 65.11 & 75.55 & 88.77 & 18.28 & 10.60 & 62.46 & 51.22 \\
opt-6.7b & prompt & c4 & 26 & --- & 27.90 & 64.39 & 48.95 & 65.84 & 75.85 & \textbf{89.83} & 18.41 & 10.83 & 63.06 & 51.67 \\
opt-6.7b & prompt & c4 & 50 & --- & 28.58 & 64.66 & \textbf{49.05} & 65.66 & 75.85 & 89.73 & 18.84 & 10.53 & 63.22 & 51.79 \\
opt-6.7b & prompt & c4 & 100 & --- & 28.38 & 64.46 & 48.67 & 65.61 & \textbf{76.24} & 89.67 & 18.44 & 11.24 & 63.38 & 51.79 \\
opt-6.7b & lora & c4 & --- & 2 & 28.84 & 63.59 & \textbf{49.05} & 66.21 & 76.15 & 88.50 & 18.92 & 11.09 & 63.33 & 51.74 \\
opt-6.7b & lora & c4 & --- & 3 & 28.61 & 63.89 & 48.97 & \textbf{66.50} & 75.97 & 89.30 & 18.95 & 11.17 & 63.48 & 51.87 \\
opt-6.7b & lora & c4 & --- & 4 & \textbf{29.27} & 64.09 & 48.98 & 66.28 & 75.90 & 88.70 & \textbf{19.19} & \textbf{11.96} & 63.19 & \textbf{51.95} \\
\midrule
llama-7b & --- & --- & --- & --- & 37.37 & 70.75 & 53.79 & 68.83 & 76.12 & 93.40 & 31.48 & 15.75 & 66.06 & 57.06 \\
% llama-7b & prompt & c4 & 3 & --- & 37.26 & 70.51 & 53.88 & 69.21 & 76.64 & 92.93 & 31.91 & 17.06 & 66.38 & 57.31 \\
llama-7b & ptune & c4 & 12 & --- & 35.55 & 70.10 & 53.39 & 66.18 & 75.73 & 91.50 & 30.35 & 15.45 & 63.01 & 55.70 \\
llama-7b & ptune & c4 & 25 & --- & 34.61 & 68.21 & 52.99 & 65.26 & 75.19 & 91 & 29.80 & 15.39 & 63.64 & 55.12 \\
llama-7b & ptune & c4 & 50 & --- & 35.21 & 67.68 & 52.77 & 64.68 & 75.19 & 90.37 & 27.28 & 11.86 & 63.75 & 54.31 \\
llama-7b & prompt & c4 & 26 & --- & 36.86 & 70.68 & 54.38 & 69.09 & 76.37 & 93 & 32.20 & 16.24 & 66.54 & 57.26 \\
llama-7b & prompt & c4 & 50 & --- & 37.66 & \textbf{71.52} & 54.48 & 69.27 & 76.46 & \textbf{93.47} & 32.44 & 17.54 & 66.93 & 57.75 \\
llama-7b & prompt & c4 & 100 & --- & \textbf{37.57} & 71.49 & 54.51 & 69.77 & 76.81 & 93.27 & 33.04 & 17.44 & 67.01 & 57.88 \\
llama-7b & lora & c4 & --- & 2 & 36.64 & 70.45 & \textbf{54.56} & 70.06 & 76.85 & 92.97 & 34.02 & \textbf{18.05} & 67.19 & 57.87 \\
llama-7b & lora & c4 & --- & 3 & 37.03 & 70.84 & 54.52 & \textbf{70.20} & 76.66 & 92.75 & 34.38 & 17.46 & 67.21 & 57.89 \\
llama-7b & lora & c4 & --- & 4 & 36.88 & 70.64 & 54.39 & 70.17 & \textbf{76.94} & 92.95 & \textbf{34.68} & 17.64 & \textbf{67.24} & \textbf{57.95} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:c4}

\end{table}


==> tables/gptq_ptb.tex <==
\begin{table}
\caption{CoreEn9 average accuracy across three separate runs for various adaptation method of 3 bit GPTQ quantized models}
\begin{tabular}{lllllrrrrrrrrrr}
\toprule
model & Peft-type & Peft-task & Prompt-tokens & Lora-r & arc_challenge & arc_easy & hellaswag & lambada_openai & piqa & sciq & triviaqa & webqs & winogrande & avg_acc \\
\midrule
facebook-opt-6.7b & ptune & ptb & 12.00 & N/A & 21.62 & 30.78 & 32.09 & 16.90 & 58.43 & 54.57 & 0.11 & 0.05 & 51.86 & 29.60 \\
facebook-opt-6.7b & ptune & ptb & 25.00 & N/A & 20.94 & 35.16 & 33.66 & 21.23 & 59.72 & 67.07 & 0.11 & 0.13 & 50.57 & 32.06 \\
facebook-opt-6.7b & prompt & ptb & 26.00 & N/A & 23.84 & 43.71 & 41.26 & 45.32 & 68.06 & 82.43 & 3.96 & 0.69 & 58.46 & 40.86 \\
facebook-opt-6.7b & prompt & ptb & 50.00 & N/A & 22.81 & 39.49 & 33.10 & 22.67 & 63.91 & 81.30 & 7.64 & 1.36 & 55.14 & 36.38 \\
facebook-opt-6.7b & ptune & ptb & 50.00 & N/A & 22.07 & 32.08 & 31.06 & 14.35 & 60.01 & 60.90 & 0.09 & 0.13 & 49.20 & 29.99 \\
facebook-opt-6.7b & prompt & ptb & 100.00 & N/A & 23.72 & 40.85 & 35.01 & 33.27 & 65.43 & 80.63 & 8.03 & 1.51 & 53.75 & 38.02 \\
huggyllama-llama-7b & ptune & ptb & 12.00 & N/A & 22.92 & 28.32 & 26.88 & 6.89 & 53.83 & 54.67 & 0.02 & 0.00 & 49.14 & 26.96 \\
huggyllama-llama-7b & ptune & ptb & 25.00 & N/A & 21.19 & 26.42 & 25.86 & 1.91 & 53.14 & 44.20 & 0.00 & 0.00 & 49.67 & 24.71 \\
huggyllama-llama-7b & prompt & ptb & 26.00 & N/A & 25.17 & 38.43 & 42.19 & 6.09 & 57.56 & 61.40 & 0.18 & 0.00 & 56.27 & 31.92 \\
huggyllama-llama-7b & prompt & ptb & 50.00 & N/A & 23.43 & 43.57 & 43.15 & 18.65 & 62.08 & 76.03 & 1.18 & 0.52 & 58.33 & 36.33 \\
huggyllama-llama-7b & ptune & ptb & 50.00 & N/A & 20.48 & 26.46 & 25.95 & 3.47 & 53.01 & 50.93 & 0.01 & 0.00 & 51.25 & 25.73 \\
huggyllama-llama-7b & prompt & ptb & 100.00 & N/A & 26.20 & 48.43 & 41.64 & 31.19 & 64.89 & 83.00 & 5.35 & 1.03 & 57.41 & 39.91 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/gptq_wikitext.tex <==
\begin{table}
\caption{Average accuracy from nine-tasks across three separate runs for various adaptation method of 3 bit GPTQ quantized models}
\begin{adjustbox}{width=\textwidth,center}

\begin{tabular}{lllll|rrrrrrrrr|r}
\toprule
model & type & task & tokens & r & arcC & arcE & hellaswag & lambada & piqa & sciq & triviaqa & webqs & winogrande & avg\_acc \\
\midrule
opt-6.7b & --- & --- & --- & --- & 29.10 & 63.76 & 48.44 & 64.60 & \textbf{75.35} & 88.40 & 17.88 & 8.32 & \textbf{64.88} & 51.19 \\

opt-6.7b & ptune & wikitext & 12 & --- & 29.15 & 61.24 & 47.95 & 62.60 & 74.27 & 86.90 & 17.84 & 9.71 & 60.17 & 49.98 \\
opt-6.7b & ptune & wikitext & 25 & --- & \textbf{29.52} & 61.93 & 48.22 & 63.52 & 74.61 & 87.53 & 18.43 & 9.09 & 60.40 & 50.36 \\
opt-6.7b & ptune & wikitext & 50 & --- & 28.96 & 62.08 & 48.35 & 63.08 & 74.16 & 88.45 & 18.48 & 10.53 & 60.38 & 50.50 \\
opt-6.7b & prompt & wikitext & 26 & --- & 29.41 & 64.13 & 48.68 & 64.82 & 75.03 & 89.13 & 19.03 & 10.04 & 61.64 & 51.32 \\
opt-6.7b & prompt & wikitext & 50 & --- & \textbf{29.52} & \textbf{63.79} & \textbf{48.69} & \textbf{65.24} & 75.08 & 88.33 & \textbf{19.32} & \textbf{11.32} & 62.61 & \textbf{51.55} \\
opt-6.7b & prompt & wikitext & 100 & --- & 28.50 & 62.16 & 48.10 & 62.54 & 74.09 & \textbf{89.43} & 19.02 & 10.51 & 61.88 & 50.69 \\
opt-6.7b & lora & wikitext & --- & 2 & 28.24 & 59.58 & 45.47 & 51.84 & 71.22 & 85.07 & 13.44 & 7.00 & 58.06 & 46.66 \\
opt-6.7b & lora & wikitext & --- & 3 & 28.30 & 57.31 & 44.39 & 48.42 & 69.95 & 83.27 & 12.11 & 7.68 & 57.30 & 45.41 \\
opt-6.7b & lora & wikitext & --- & 4 & 28.55 & 57.07 & 43.95 & 48.10 & 69.44 & 83.80 & 12.03 & 8.30 & 57.38 & 45.40 \\
\midrule
llama-7b & --- & --- & --- & --- & 37.71 & 71.46 & 53.11 & 68.58 & \textbf{76.01} & 92.60 & 33.02 & 17.96 & 67.48 & 57.55 \\
% llama-7b & prompt & wikitext & 3 &  & 37.31 & 71.37 & 53.75 & 69.43 & 75.52 & 92.70 & 31.25 & 18.34 & 66.72 & 57.38 \\
llama-7b & ptune & wikitext & 12 & --- & 34.81 & 69.38 & 52.54 & 65.42 & 74.83 & 89.70 & 30.63 & 16.54 & 62.56 & 55.16 \\
llama-7b & ptune & wikitext & 25 & --- & 35.01 & 69.11 & 52.27 & 65.03 & 74.23 & 89.53 & 29.17 & 15.58 & 62.98 & 54.77 \\
llama-7b & ptune & wikitext & 50 & --- & 33.70 & 66.25 & 51.84 & 64.01 & 73.53 & 88 & 26.69 & 14.10 & 62.95 & 53.45 \\
llama-7b & prompt & wikitext & 26 & --- & 37.97 & 72.17 & 53.73 & 69.31 & 75.60 & \textbf{92.90} & 33.56 & 20.11 & 67.01 & 58.04 \\
llama-7b & prompt & wikitext & 50 & --- & 37.91 & 71.66 & 53.99 & \textbf{69.73} & 75.86 & 92.27 & 34.26 & 20.22 & \textbf{67.75} & 58.18 \\
llama-7b & prompt & wikitext & 100 & --- & \textbf{38.51} & \textbf{72.19} & \textbf{54.38} & 69.20 & 75.95 & 92.17 & \textbf{34.37} & \textbf{21.18} & 67.19 & \textbf{58.35} \\
llama-7b & lora & wikitext & --- & 2 & 33.96 & 65.03 & 49.36 & 45.35 & 70.58 & 87.15 & 22.06 & 10.93 & 59.08 & 49.28 \\
llama-7b & lora & wikitext & ---  & 3 & 34.07 & 64.31 & 48.04 & 43.45 & 69.68 & 83.53 & 20.05 & 10.42 & 59.61 & 48.13 \\
llama-7b & lora & wikitext & ---  & 4 & 35.16 & 63.45 & 47.65 & 39.81 & 68.65 & 81.85 & 20.19 & 9.46 & 59.47 & 47.30 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:wiki}
\end{table}


==> tables/latency_table.tex <==


\begin{table}[h]
\caption{The average run-time on CPU and GPU of for different fine tuning methods. "Q" indicates 3-bit quantization by GPTQ}
\begin{tabular}{llllllrr}
\toprule
Model &	Peft type & config & num param &batch &	seq & cpu-time & gpu-time \\
\midrule
LLama7b	&&&0&	16 &1024&	2.397&	1.858 \\
QLLama7b&&&0&	16 &1024&	3.394&	2.18 \\
QLLama7b& prompt &	26 tokens&	106496&	16&	1024&	3.547&	2.417\\
QLLama7b& prompt &	50 tokens&	204800&	16&	1024&	3.6&	2.462\\
QLLama7b& prompt & 100 tokens&	409600&	16&	1024&	3.748&	2.546\\
QLLama7b& lora   &	r=4&	8945664&	16&	1024&	3.889&	2.8\\
\bottomrule
\end{tabular}
\label{tab:latency}
\end{table}

==> tables/sparsegpt_c4.tex <==
\begin{table}
\caption{Average accuracy across three separate runs for various adaptation method of sparseGPT compressed models at $50\%$}
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{lllll|rrrrrrrrr|r}
\toprule
model & type & task & tokens & r & arcC & arcE & hellaswag & lambada & piqa & sciq & triviaqa & webqs & winogrande & avg\_acc \\
\midrule
opt-6.7b & --- & --- & --- & --- & 28.41 & 63.01 & 47.67 & 70.56 & 75.19 & 89.40 & 17.79 & 9.69 & 63.93 & 51.74 \\
opt-6.7b & ptune & c4 & 12 & --- & 27.30 & 61.52 & 47.45 & 63.64 & 75.05 & 88.50 & 16.81 & 7.38 & 61.33 & 49.89 \\
opt-6.7b & ptune & c4 & 25 & --- & 28.58 & 62.23 & 47.91 & 64.43 & 75.24 & 88.40 & 17.26 & 8.02 & 61.85 & 50.44 \\
opt-6.7b & ptune & c4 & 50 & --- & 28.21 & 62.46 & 48.01 & 65.35 & 75.33 & 88.70 & 17.37 & 7.50 & 61.88 & 50.53 \\
opt-6.7b & prompt & c4 & 26 & --- & 28.78 & 63.36 & 48.34 & 68.44 & 75.34 & 90.30 & 18.80 & 12.22 & 63.27 & 52.09 \\
opt-6.7b & prompt & c4 & 50 & --- & 29.18 & 63.50 & 48.38 & 68.04 & 75.17 & 90.00 & 19.01 & 12.65 & 63.38 & 52.15 \\
opt-6.7b & prompt & c4 & 100 & --- & 28.93 & 63.67 & 48.43 & 67.49 & 75.33 & 89.77 & 18.92 & 12.96 & 63.09 & 52.06 \\
opt-6.7b & lora & c4 & --- & 2 & 29.52 & 63.71 & 48.66 & 66.63 & 75.72 & 88.57 & 18.42 & 9.70 & 63.72 & 51.63 \\
opt-6.7b & lora & c4 & --- & 3 & 29.24 & 63.52 & 48.72 & 66.60 & 75.79 & 88.53 & 18.60 & 9.81 & 64.30 & 51.68 \\
opt-6.7b & lora & c4 & --- & 4 & 29.58 & 63.22 & 48.71 & 66.73 & 75.39 & 88.27 & 18.78 & 9.53 & 64.93 & 51.68 \\
\midrule
llama-7b & --- & --- & --- & --- & 37.03 & 70.33 & 51.68 & 74.54 & 77.04 & 93.50 & 28.88 & 14.07 & 68.03 & 57.23 \\
llama-7b & ptune & c4 & 12 & --- & 32.38 & 63.38 & 50.05 & 64.88 & 72.66 & 88.60 & 24.27 & 11.12 & 57.22 & 51.62 \\
llama-7b & ptune & c4 & 25 & --- & 33.85 & 66.13 & 50.38 & 65.31 & 74.30 & 88.83 & 23.72 & 11.06 & 59.41 & 52.55 \\
llama-7b & ptune & c4 & 50 & --- & 31.85 & 65.14 & 49.95 & 64.16 & 74.17 & 87.40 & 20.31 & 8.17 & 59.56 & 51.19 \\
llama-7b & prompt & c4 & 26 & --- & 38.28 & 70.86 & 53.59 & 71.42 & 77.04 & 92.57 & 29.67 & 15.37 & 67.03 & 57.32 \\
llama-7b & prompt & c4 & 50 & --- & 37.86 & 70.72 & 53.73 & 71.70 & 77.15 & 92.17 & 30.35 & 14.29 & 67.17 & 57.24 \\
llama-7b & prompt & c4 & 100 & --- & 38.25 & 71.54 & 53.93 & 71.10 & 77.11 & 92.50 & 30.63 & 14.71 & 67.19 & 57.44 \\
llama-7b & lora & c4 & --- & 2 & 37.80 & 70.42 & 53.98 & 71.16 & 77.01 & 91.87 & 33.01 & 14.45 & 67.09 & 57.42 \\
llama-7b & lora & c4 & --- & 3 & 37.23 & 70.38 & 53.92 & 71.02 & 76.95 & 92.17 & 32.62 & 14.80 & 67.59 & 57.41 \\
llama-7b & lora & c4 & --- & 4 & 38.05 & 70.49 & 53.88 & 71.17 & 77.17 & 92.03 & 32.94 & 14.84 & 67.74 & 57.59 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/sparsegpt_ptb.tex <==
\begin{table}
\caption{Average accuracy across three separate runs for various adaptation method of sparseGPT compressed models at 50%}
\begin{tabular}{lllllrrrrrrrrrr}
\toprule
model & Peft-type & Peft-task & Prompt-tokens & Lora-r & arc_challenge & arc_easy & hellaswag & lambada_openai & piqa & sciq & triviaqa & webqs & winogrande & avg_acc \\
\midrule
\bottomrule
\end{tabular}
\end{table}


==> tables/sparsegpt_wikitext.tex <==
\begin{table}
\caption{Average accuracy across three separate runs for various adaptation method of sparseGPT compressed models at $50\%$}
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{lllll|rrrrrrrrr|r}
\toprule
model & type & task & tokens & r & arcC & arcE & hellaswag & lambada & piqa & sciq & triviaqa & webqs & winogrande & avg\_acc \\
\midrule
opt-6.7b & --- & --- & --- & --- & 27.47 & 63.47 & 46.48 & 66.80 & 73.99 & 88.70 & 20.30 & 12.06 & 63.93 & 51.47 \\
opt-6.7b & ptune & wikitext & 12 & --- & 28.70 & 61.62 & 46.34 & 62.10 & 72.49 & 86.77 & 18.81 & 11.99 & 60.30 & 49.90 \\
opt-6.7b & ptune & wikitext & 25 & --- & 28.98 & 62.36 & 46.69 & 62.72 & 72.83 & 86.70 & 19.57 & 11.98 & 60.72 & 50.28 \\
opt-6.7b & ptune & wikitext & 50 & --- & 29.38 & 61.46 & 47.02 & 63.16 & 73.50 & 87.50 & 19.49 & 13.04 & 60.96 & 50.61 \\
opt-6.7b & prompt & wikitext & 26 & --- & 29.21 & 63.29 & 46.73 & 66.06 & 73.52 & 90.40 & 20.35 & 12.49 & 62.46 & 51.61 \\
opt-6.7b & prompt & wikitext & 50 & --- & 29.13 & 63.78 & 47.11 & 66.04 & 73.72 & 89.47 & 20.47 & 13.27 & 63.06 & 51.78 \\
opt-6.7b & prompt & wikitext & 100 & --- & 29.29 & 63.79 & 47.21 & 65.74 & 73.81 & 90.30 & 20.67 & 13.01 & 62.41 & 51.80 \\
opt-6.7b & lora & wikitext & --- & 2 & 28.16 & 59.47 & 44.52 & 49.72 & 69.98 & 84.60 & 13.68 & 8.45 & 57.40 & 46.22 \\
opt-6.7b & lora & wikitext & --- & 3 & 27.13 & 57.48 & 43.77 & 46.91 & 69.37 & 84.07 & 12.04 & 7.51 & 57.62 & 45.10 \\
opt-6.7b & lora & wikitext & --- & 4 & 28.50 & 56.99 & 43.50 & 45.03 & 68.59 & 84.73 & 12.22 & 7.76 & 57.27 & 44.95 \\
\midrule
llama-7b & --- & --- & --- & --- & 37.97 & 69.87 & 50.75 & 71.32 & 75.08 & 93.10 & 30.58 & 15.75 & 67.56 & 56.89 \\
llama-7b & ptune & wikitext & 12 & --- & 29.31 & 57.59 & 48.49 & 59.64 & 68.50 & 85.50 & 23.24 & 9.23 & 53.87 & 48.37 \\
llama-7b & ptune & wikitext & 25 & --- & 30.26 & 62.03 & 49.68 & 61.41 & 70.68 & 85.77 & 24.44 & 11.88 & 57.72 & 50.43 \\
llama-7b & ptune & wikitext & 50 & --- & 31.17 & 62.99 & 49.69 & 61.08 & 71.91 & 86.30 & 23.20 & 10.99 & 57.85 & 50.58 \\
llama-7b & prompt & wikitext & 26 & --- & 36.86 & 70.02 & 53.03 & 69.28 & 75.30 & 91.87 & 31.68 & 17.01 & 65.46 & 56.72 \\
llama-7b & prompt & wikitext & 50 & --- & 36.63 & 70.30 & 53.32 & 68.72 & 75.34 & 91.73 & 32.18 & 16.49 & 65.75 & 56.72 \\
llama-7b & prompt & wikitext & 100 & --- & 37.29 & 70.69 & 53.39 & 68.71 & 75.39 & 91.80 & 31.70 & 16.44 & 64.85 & 56.69 \\
llama-7b & lora & wikitext & --- & 2 & 34.58 & 61.62 & 47.17 & 40.97 & 69.15 & 87.03 & 21.02 & 10.57 & 57.41 & 47.72 \\
llama-7b & lora & wikitext & --- & 3 & 32.71 & 61.95 & 45.79 & 39.13 & 68.75 & 84.07 & 18.93 & 8.79 & 57.54 & 46.41 \\
llama-7b & lora & wikitext & --- & 4 & 32.91 & 61.88 & 45.03 & 38.40 & 68.21 & 84.73 & 18.49 & 7.50 & 57.48 & 46.07 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

